User-oriented Natural Human-Robot Control with Thin-Plate Splines and LRCN

We propose a real-time vision-based teleoperation approach for robotic arms that employs a single depth-based camera, exempting the user from the need for any wearable devices. By employing a natural user interface, this novel approach leverages the conventional fine-tuning control, turning it into a direct body pose capture process. The proposed approach is comprised of two main parts. The first is a nonlinear customizable pose mapping based on Thin-Plate Splines (TPS), to directly transfer human body motion to robotic arm motion in a nonlinear fashion, thus allowing matching dissimilar bodies with different workspace shapes and kinematic constraints. The second is a Deep Neural Network hand-state classifier based on Long-term Recurrent Convolutional Networks (LRCN) that exploits the temporal coherence of the acquired depth data. We validate, evaluate and compare our approach through both classical cross-validation experiments of the proposed hand state classifier; and user studies over a set of practical experiments involving variants of pick-and-place and manufacturing tasks. Results revealed that LRCN networks outperform single image Convolutional Neural Networks; and that users' learning curves were steep, thus allowing the successful completion of the proposed tasks. When compared to a previous approach, the TPS approach revealed no increase in task complexity and similar times of completion, while providing more precise operation in regions closer to workspace boundaries.

==> experiments.tex <==
\section{\textbf{Practical 
experiments}}
\label{sec:practical_experiments}

To validate and compare the proposed Thin Plate Splines Pose Mapping (TPS-PM, Sections~\ref{sec:tps} and \ref{sec:customtps}) to the previously proposed Naive Affine Pose Mapping (NA-PM, Section~\ref{sec:naivemapping}), performed usability tests to measure the user experience with both compared approaches. We set up a test environment and predetermined a set of five tasks in which users were asked to manipulate objects with the robotic arm through both pose mapping approaches.

For each position mapping approach, the following aspects were evaluated:
\begin{itemize}
    \item \textbf{Goal achievement}. Were users able to accomplish the required tasks?
    \item \textbf{Comfort}. Which approach feels more comfortable and natural?
    \item \textbf{Learning curve}. Does the learning curve allow rapid progress in such a way that users could cope with increasingly difficult tasks?
\end{itemize}

The set of tasks required not only motor skills and spatial awareness from the users but also the ability to adapt to the specific transformation being used. Each experiment has some increased difficulty in relation to the previous one. Before the experiments, users were asked to fill out a compliance form allowing them to be recorded during the sections for analysis and scientific purposes. The elements employed in the experiments are:
\begin{itemize}
    \item two cubes of length equal to 5 cm;
    \item a cylindrical platform with a red-marked open-bottom of 10 cm diameter and a height of 12 cm. The top has 7.5 cm of diameter.
\end{itemize}

When the platform was placed upside-down, it became a hoop. We also defined 4 areas within the robot workspace, named from A to D.

To quantify each task, we use the concept of atomic movements. One atomic movement is an indivisible continuous displacement of the robot gripper with well-defined starting and ending times. Translations and gripper state variations (opening/closing, or grab/release) are considered atomic movements. Thus, each task can be performed using a minimum number of atomic movements.

More specifically, experiments were:

\begin{enumerate}
    \item \textbf{Take a cube from region B to region A}. It's an initial task to test the user's ability to successfully grab and move an object to another location. Can be achieved with a minimum of 4 atomic movements: home-to-B, grab, B-to-A, release.
    \item \textbf{Swap cubes between regions B and A, using region C as auxiliary}. The purpose of this task is to measure the increase in user's skills since the first task. The swap task can be done in a minimum of 12 atomic movements, all of them with the same difficulty as the first task, e.g.: home-to-A, grab, A-to-C, release, C-to-B, grab, B-to-A, release, A-to-C, grab, C-to-B, release.
    \item \textbf{Bring cubes from regions A and B to the hoop}. This task introduces the necessity of motion at higher heights, thus increasing task complexity in the vertical axis. Users have to take into consideration avoiding collision between the gripper and the hoop while bringing the cubes to the proper height before releasing it. Skills evaluated here also include ease of use near robot boundaries, since the platform is located at region D. It can also be executed with a minimum of 8 atomic movements, e.g: home-to-A, grab, A-to-hoop, release, hoop-to-B, grab, B-to-hoop, release.
    \item \textbf{Pile cubes in region A}. This task introduces a new component in evaluation which is the ability to fine-tune the cube position to successfully pile one cube onto another. Previous tasks had a less strict acceptance with relation to where the cubes might be placed. Can also be performed within 8 atomic movements, e.g.: home-to-C, grab, C-to-A, release, A-to-B, grab, B-to-A, release.
    \item \textbf{Move a cube from platform to A, then from B to platform.} Skills needed are boundary regions control and the ability to fine-tune the cube position to place it on top of the platform. Can also be performed on a minimum of 8 atomic movements, e.g.: home-to-hoop, grab, hoop-to-A, release, A-to-B, grab, B-to-hoop, release.
\end{enumerate}

\begin{figure}[!b]
\centering \includegraphics[width=\columnwidth]{fig/experiment_photos_v2_cor.png}\\
\caption{Practical experiment workspaces, showing the initial (left) and goal (right) states. Each row represents one experiment from 1 to 5, respectively.}
\label{fig:experiments}
\end{figure}

Starting and goal configurations for each of the previously discussed experiments are shown in Fig.~\ref{fig:experiments}. In order to measure time completion for each experiment, we defined the following conditions: (1) time counter starts as soon as the user-control mode is triggered, and; (2) time counter finishes as soon as the goal is reached and the objects of interaction remain still. Success occurs when the goal is reached and objects stay within established areas (not touching the workspace region outside the black markers). A fail occurs when the experiment reaches a state where the goal is not possible to be achieved without human assistance (i.e. when one cube falls outside the robot workspace). 

The previously discussed set of five experiments was repeated twice for each user, firstly using the Homogeneous Transformation discussed in \ref{sec:ht} and then using the Thin Plate Spline mapping discussed in \ref{sec:tps}. Before the very first experiment of each set started, a ``playground time'' of two minutes was given to each user for free operation so that they could acquire familiarity with the transformation mapping. After the very last experiment of each session, users were asked to answer two multiple choices qualitative questions by selecting a value in the range from 1 to 5, about how they felt with relation to the used mapping:
\begin{itemize}
    \item \textbf{(Q1) How smooth was the movement of the robotic arm during control?} This question evaluates how comfortable users were with the smoothness of the robotic arm movement when his right hand moves. %A smooth movement would mean a rate $d_R/d_U$ of approximately $1$. A rough movement would have larger values, meaning that a small hand displacement would lead to a big robot displacement.
    \item \textbf{(Q2) How difficult was the movement near robot boundaries?} This question evaluates the consistency of the mapping when the robot gripper gets closer to its boundaries. A good mapping would present the user with a consistent low difficulty that does not depend on the region of operation, with an overall effort being as minimum as possible.
\end{itemize}

After both sets of experiments were finished and their respective objective questions were answered, the users were asked to answer a set of 3 discursive questions to evaluate overall opinion about the comparison between both mappings:

\begin{itemize}
    \item \textbf{(Q3) In your opinion, which were the advantages of each mapping?}
    \item \textbf{(Q4) What were the challenges found during the experiment?}
    \item \textbf{(Q5) Would you have any suggestions to improve future experiences?}
\end{itemize}

All participant answers were collected through an online form for posterior analysis. At this phase, five participants volunteered for testing purposes.
